Snowmass Topical Report: Underground Facilities for Neutrinos

This topical report of the 2021 US Community Study on the Future of Particle Physics (Snowmass 2021) summarizes the underground facilities needs for upcoming and next generation neutrino experiments. The underground facilities needs are discussed in the context of two broad categories: accelerator neutrinos, in particular with respect to the Deep Underground Neutrino Experiment (DUNE); and non-accelerator neutrinos, focusing on neutrinos from natural sources and on searches for neutrinoless double-beta decay.

==> Underground/Header.tex <==
%JLO% -- The next line needs to be removed
\chapter*{}

  \vfill

\begin{center}
\begin{Huge}   {\bf  TOPICAL GROUP REPORTS}

\bigskip

\bigskip

 {\bf Underground Facilities}
 %JLO% -- The next line needs to be removed
 \addcontentsline{toc}{chapter}{Underground Facilities}

\vfill

\vfill

\end{Huge}
\end{center}

\newpage
\thispagestyle{empty}
\mbox{\null}




==> Underground/Underground.tex <==

\setcounter{chapter}{9} 

\chapter{Underground Facilities Executive Summary}

\authorlist{L.~Baudis, J.~Hall, K.~Lesko, J.L.~Orrell}
{T.~Bolton, J.~Cooley$^*$, E.~Dahl$^*$, M.P.~Decowski, A.~De~Roeck$^*$, S.~Hertel, A.~Kamaha, H.~Lippincott$^*$, B.~Mount, K.~Ni, G.~Orebi~Gann$^*$, E.~Pantic, D.~Robertson, R.~Schnee, D.~Speller \newline \textit{$^*$Liaisons from other Snowmass Frontiers.} }

\section{Introduction}

From the properties and nature of the neutrino to the search for direct measurement of the dark matter, research performed at underground facilities tackles the collection of precision knowledge of the constituents of the Standard Model of particle physics to broadly open-ended search well Beyond the Standard Model (BSM). The preceding chapters and reports from other Frontiers layout the science case for these and other avenues of particle physics research. Here we identify the needs and requirements for underground facilities to continue support the breadth of particle physics research planned in the coming 10-15 years.

\subsection{Taking stock from Snowmass 2013}

The Underground Laboratory Capabilities report from Snowmass 2013~\cite{10.48550/arxiv.1401.6115} outlines plans, needs, and concerns contemporary at that time. Here we briefly take stock of what has been accomplished, or in some cases, side-stepped in the progress toward science performed in underground facilities.

\textit{The following is in draft; the bullets will be wrapped.}

\begin{itemize}
    \item Then: Identification and creation of new underground labs: SNOLAB, JinPing (CJPL), Canfranc (LSC), and Sanford (SURF)
    \begin{itemize}
        \item Now: These underground labs have been in operation continually and continue to expand to support underground research.
    \end{itemize}
    \item Then: Expansions of existing international labs CJPL, JUNO, RENO50 and Yangyang, Kamioka for Hyper-K, Modane, India Neutrino Observatory (INO), ANDES (South America), CUPP (Finland). [MPD: Boulby expansion?]
    \begin{itemize}
        \item Now: All of these efforts, except for \ldots, have moved forward in the decade after 2013. [LB: should we be more concrete? Some - for instance Yangyang - were not technically expanded, but new labs were built, in this case Yemilab; MPD:Hyper-K is not in the old Kamioka mine, but a new lab]
    \end{itemize}
    \item Then: Expansion plans of existing U.S. underground labs KURF, Soudan, SURF, WIPP.
    \begin{itemize}
        \item Now: Soudan has closed. KURF has a measurement lab at 300 m.w.e. and is developing a 700 m.w.e. deep location; the 1475 m.w.e. location is currently closed (See Letter of Interest: SNOWMASS21-UF1\_UF4-RF4\_RF3\_ODonnell-007). DMTPC is the most recently active particle physics experiment active at WIPP [LB: is it still running?]. SURF has become the primary focal point for deep underground science within the U.S.
    \end{itemize}
    \item Then: 
    \begin{itemize}
        \item Now: 
    \end{itemize}
    \item Then: 
    \begin{itemize}
        \item Now: 
    \end{itemize}
    \item Then: 
    \begin{itemize}
        \item Now: 
    \end{itemize}
    \item Then: 
    \begin{itemize}
        \item Now: 
    \end{itemize}
    \item Then: 
    \begin{itemize}
        \item Now: 
    \end{itemize}
    \item Then: 
    \begin{itemize}
        \item Now: 
    \end{itemize}
\end{itemize}




\subsection{Evolving landscape}

New labs: Australia




\section{Key Observations from Underground Facilities \& Infrastructure Topical Reports}

\subsection{Underground Facilities for the Neutrinos}
\textit{Summarize the key points from UF1}

 Preservation of competitiveness in the US neutrino program is dependent on future access to clean, deep underground space.  Planning for future needs must begin now.
 Local, expert support at underground facilities is critical for success.There is strong community support for better user facility support for international collaborators.
 
 There is a need for central coordination of resources, including radio assay capabilities, low-background counting, data for cosmogenic activation, radiopurity databases, and shared data and simulations, perhaps by one of the underground laboratories.
 
  Future experiments and successful R\&D should plan for additional supporting facilities such as space for prototypes, R\&D etc.  A need for cryogenic facilities has strong synergies with dark matter and quantum information science.


 


 Plans to pursue neutrino science beyond the tonne-scale \ndbd program require inter-agency planning efforts for future underground facilities, particularly with respect to the preparation and allocation of deep underground space.



As referenced in the 2013 report \cite{U1-css2013ulc}, depth requirements for neutrino and dark matter experiments depends on which technology is employed.  In keeping with the several avenues of research and development currently being pursued by \ndbd experiments, simulations corresponding to suitable combinations in each major category (e.g. detector substrate, sensor, etc) may also inform whether current depth and experimental space  constraints require more concentrated development of a particular technology for a planned experiment to be sited, or if underground facilities must be expanded.


\subsection{Underground Facilities for the Cosmic Frontier}
\textit{Summarize the key points from UF2}

Multiple new underground dark matter experiments are expected and being planned (at both large and small scales).   At the same time, underground facilities are largely subscribed by existing projects, with only very limited space available in the coming years.  There is, then, a clear need for additional underground space, tailored to the needs of dark matter experiments.

This underground space should specifically include
Both large spaces for large experiments (liquid noble) and small spaces for smaller experiments (cryogenic bolometer, ‘other’).  The assembly of large liquid noble experiments will occur largely in the underground environment, meaning they require large underground radon-free clean rooms.  Given the volume of gas/cryogen, such experiments also require large underground areas for staging (e.g., gas storage) and experiment utilities (e.g. pumps, distillation).

These new suitable spaces must be available by the late 2020's to meet the demand.  This demand may be met in North America by proposed new excavations at SURF or SNOLab.


\subsection{Supporting Capabilities for Underground Science}
\textit{Summarize the key points from UF4}

Future, larger experiments will increasingly require underground assembly with stricter radioactivity requirements.  There will need to be larger, cleaner cleanrooms, often with better radon-reduction systems and increased monitoring capabilities for ambient contaminants.   
Methods to assay radon-daughter plate-out will need to be improved. There will be increased need for underground machine shops. 

Most assay needs may be met by existing worldwide capabilities with organized cooperation between facilities and experiments. Improved assay sensitivity is needed for assays of bulk and surface radioactivity for some materials for some experiments, and would be highly beneficial for radon emanation.  



\subsection{Underground Detectors \& Synergistic Research}
\textit{Summarize the key points from UF3/5}

A variety of research beyond high energy physics is performed in underground laboratories. These research activities from other disciplines include burgeoning R\&D in quantum information science, accelerator-based nuclear astrophysics, tests of fundamental symmetries, gravitational wave detection, and geology \& geophysics.

In most all cases, research groups from differing disciplines are able to work in shared underground facility space harmoniously and in some cases synergistically. Smaller-scale research efforts benefit substantially from the investment in underground facilities and infrastructure initially prepared for larger-scale science endeavors.

Evaluating the ``total research impact'' of shared-usage underground research facilities should take into account the full disciplinary breadth of research performed.


\subsection{Underground Facilities \& Infrastructure}
\textit{Summarize the key points from UF6}

\section{Outlook}



\section{Conclusion \& Recommendations}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%  If you would like to use BibTEX for the bibliography, please feel free to do so.  It is not required.

%  To use BibTeX,

%    1.  uncomment the following two lines,
%    2.  comment out everything below from  \begin{thebibliography}{99}   to \end{thebibliography).
%    3.  create the file  myreferences.bib in this directory, and process this file in the usual way

%\bibliographystyle{JHEP}
%\bibliography{Underground/myreferences} 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\begin{thebibliography}{99}

\input Underground/bibliography.tex

\end{thebibliography}

==> Underground/bibliography.tex <==


\bibitem{U-Scoresby}
J. Scoresby, ``Journals'', 1820.

\bibitem{U-Beale}
A. Beale, ``Surgical Writings'', 1839.

\bibitem{hvkk00}
H. V. Klapdor-Kleingrothaus, ``From the Early Days until the Gauge Theory Era'', \textit{Sixty Years of Double Beta Decay}, 2000

\bibitem{10.48550/arxiv.1401.6115}
Gilchriese, M. G. and Cushman, P. and Heeger, K. and Klein, J. and Scholberg, K. and Sobel, H. and Witherell, M., \textit{Planning the Future of U.S. Particle Physics (Snowmass 2013): Chapter 7: Underground Laboratory Capabilities}, arXiv:1401.6115, (2014).




==> tcilcomm.tex <==
% Macros used for TCI styles released with Scientific Word 1.1.
%Copyright (C) 1992-93 TCI Software Research, Inc.
\typeout{TCILCOMM Macros for TCI styles <08 Apr 93>.}
%
% Revisions:
% 08 Apr 93 - GP change line length to under 80 characters
% 30 Mar 92 - AO added \setmoremathsizes and hooks to, e.g. \@xpt,
%             for support of bold Greek
%
%%ltg added this to try to get 12pt to come through
%\DeclareOption{12pt}{\renewcommand\@ptsize{2}}
%%end ltg

\def\@ptoptions{%
 \let\@elt\relax\@for\@tempa:=\@optionlist\do{%
  \expandafter\let\expandafter\@tempb\csname ds@\@tempa\endcsname
  \expandafter\let\expandafter\@tempc\csname ds@11pt\endcsname
  \ifx\@tempb\@tempc\else
   \expandafter\let\expandafter\@tempc\csname ds@12pt\endcsname
   \ifx\@tempb\@tempc\else\let\@tempb\relax\fi
   \fi
  \@tempb
  }%
 }%
%
% read in style file, but only process the pt size options
%
\def\@ptoptinput#1{%
 \let\@save@optionlist\@optionlist
 \let\@save@options\@options
 \let\@options\@ptoptions
 %
 \input #1
 %
 \let\@optionlist\@save@optionlist
 \let\@options\@save@options
 }%
%
% the <21 Feb 92> version of letter.sty requires:
\ifx\undefined\reset@font
 \def\reset@font{}%
 \fi
%
% Change LaTeX
%
% Add command to append tokens
\newtoks\@temptokenb
\long\def\appdef#1#2{%
 \ifx#1\undefined\let#1\@empty\fi
 \@temptokena\expandafter{#1}\@temptokenb{#2}%
 \edef#1{\the\@temptokena\the\@temptokenb}%
 }%
\long\def\prepdef#1#2{%
 \ifx#1\undefined\let#1\@empty\fi
 \@temptokena\expandafter{#1}\@temptokenb{#2}%
 \edef#1{\the\@temptokenb\the\@temptokena}%
 }%
% Discard contents of \box\@cclv at beginning of document
\appdef\document{{\output{\setbox\z@\box\@cclv}\endgraf\null\eject}}%
% Fix mark register expansion
\def\leftmark{\expandafter\@leftmark\botmark{}{}{}\@nil}%
\def\rightmark{\expandafter\@rightmark\firstmark{}{}{}\@nil}%
\def\@leftmark#1#2#3\@nil{#1}%
\def\@rightmark#1#2#3\@nil{#2}%
%
%\show\raggedright
\newskip\raggedglue
\raggedglue\z@ plus20\p@ minus\z@
\def\raggedright{%
 \let\\=\@centercr\@rightskip\raggedglue\rightskip
 \@rightskip\leftskip\z@\parindent\z@
 }%
%
\def\@centercr{%
 \ifhmode\unskip\else\@badcrerr\fi\@@par
 \@ifstar{\penalty\@M\@xcentercr}{\@xcentercr}%
 }%
%
\def\traceoutput{\tracingoutput2\showboxbreadth\maxdimen
 \showboxdepth\maxdimen}%
%
\newcount\@hour\newcount\@minute\chardef\@x10\chardef\@xv60
\def\@time{%
  \@minute\time\@hour\@minute\divide\@hour\@xv
  \ifnum\@hour<\@x 0\fi\the\@hour:%
  \multiply\@hour\@xv\advance\@minute-\@hour
  \ifnum\@minute<\@x 0\fi\the\@minute
  }%
%
% change \@array to allow \par to mean something within its scope
%
\def\@array [#1]#2{%
 \setbox\@arstrutbox\hbox{\vrule height\arraystretch\ht
  \strutbox depth\arraystretch\dp\strutbox width\z@}%
 \@mkpream{#2}%
 \edef\@preamble{\halign\noexpand\@halignto\bgroup\tabskip
  \z@\@arstrut\@preamble\tabskip\z@\cr}%
 \let\@startpbox\@@startpbox\let\@endpbox\@@endpbox
 \if#1t\vtop\else\if#1b\vbox\else\vcenter\fi\fi
 \bgroup
  %\let\par\relax
  \let\@sharp##
  \let\protect\relax
  \lineskip\z@\baselineskip\z@
  \@preamble
 }%
%
% Expands to hex digit corresponding to the value of the argument
%
\def\hexnumber@#1{\ifnum#1<10 \number#1\else
 \ifnum#1=10 A\else\ifnum#1=11 B\else\ifnum#1=12 C\else
 \ifnum#1=13 D\else\ifnum#1=14 E\else\ifnum#1=15 F\fi\fi\fi\fi\fi\fi\fi}%
%
% define command to set more math sizes.
% Styles like Greekbf will hook in here.
%
\def\setmoremathsizes#1#2#3{}%
%
% define size switch addenda
%  Note: these choices agree with those in lfonts.tex, even if incorrect.
%
\prepdef\@vpt{\setmoremathsizes{fiv}{fiv}{fiv}}%
\prepdef\@vipt{\setmoremathsizes{six}{six}{six}}%
\prepdef\@viipt{\setmoremathsizes{sev}{fiv}{fiv}}%
\prepdef\@viiipt{\setmoremathsizes{egt}{six}{fiv}}%
\prepdef\@ixpt{\setmoremathsizes{nin}{six}{fiv}}%
\prepdef\@xpt{\setmoremathsizes{ten}{sev}{fiv}}%
\prepdef\@xipt{\setmoremathsizes{elv}{egt}{six}}%
\prepdef\@xiipt{\setmoremathsizes{twl}{egt}{six}}%
\prepdef\@xivpt{\setmoremathsizes{frtn}{ten}{sev}}%
\prepdef\@xviipt{\setmoremathsizes{svtn}{twl}{ten}}%
\prepdef\@xxpt{\setmoremathsizes{twty}{frtn}{twl}}%
\prepdef\@xxvpt{\setmoremathsizes{twty}{twty}{svtn}}%
%
% The \newfield command defines (like \newenvironment) a user syntax:
%
%   \newfield{foo}
%
% lets you write
%
%   \begin{foo}...\end{foo}
%
% but differs from \newenvironment in that TeX parses the entire content
% of the field and stores it in a macro \the@foo, and then executes \@do@foo.
%
% This means that the content of the field is actually more like an argument
% than the content of an environment. So \verb will not necessarily work
% within a field, and neither will \index. Caveat emptor.
%
% The default procedure for a field is to process its argument within a
% group.  If you want a field to simply store its data away, define its
% procedure to be synonymous with \@empty, as illustrated below.
%
\long\def\@readenvir#1#2\end{%
 \appdef\envirsofar{#2}%
 \@ifnextchar\bgroup{\@checkenvir{#1}}{\@envirenderr}%
 }%
%
\def\@envirenderr{%
 \@latexerr{\string\end\space not followed by environment name}\@eha
 }%
%
\def\@checkenvir#1#2{%
 \def\@tempa{#1}\def\@tempb{#2}%
 \ifx\@tempa\@tempb
  \ifx\envirsofar\@blankspace\let\envirsofar\@empty\fi
  \expandafter\let\csname the@#1\endcsname\envirsofar
  \def\@tempa{\csname @do@#1\endcsname}%
  \else
  \appdef\envirsofar{\end{#2}}%
  \def\@tempa{\@readenvir{#1}}%
  \fi
 \@tempa
 }%
%
\def\newfield#1#2{%
 \expandafter\@ifdefinable\csname#1\endcsname{%
  \expandafter\def\csname#1\endcsname{%
   \endgroup\let\envirsofar\@empty\@readenvir{#1}%
   }%
  \expandafter\let\csname the@#1\endcsname\@empty
  \expandafter\ifx\csname @do@#1\endcsname\relax
   \expandafter\def\csname @do@#1\endcsname{{\csname the@#1\endcsname}}%
   \fi
  }%
 }%
%
\def\@blankspace{ }% SciWord's nil field
%
\def\letparBL{\def\par{\\}}%
\def\letparSP{\def\par{\ }}%
\def\letparQD{\def\par{\quad}}%
\def\letparSL{\def\par{\hbox to1em{\hfil/\hfil}}}%
%
% When \par is processed in the page head, gobble up the rest of the
% argument.
\def\@gobblepar#1\@empty{}%
%
% Physical page size after trim
\newdimen\trimwidth
\newdimen\trimheight
\newdimen\botmargin
\newdimen\marginpartotal
%
\def\adjustpagemargin{% adjust \oddsidemargin by \marginpartotal
 \marginpartotal\marginparwidth\advance\marginpartotal\marginparsep
 \advance\oddsidemargin\marginpartotal
 }%
%
\def\settextheight{% calculate textheight constrained by:
 \textheight\trimheight
 \advance\textheight-\topmargin
 \advance\textheight-\headheight
 \advance\textheight-\headsep
 \advance\textheight-\footskip
 \advance\textheight-\botmargin
 }%
%
\def\vcenterpagemargin{% calculate \topmargin constrained by:
 \topmargin\trimheight
 \advance\topmargin-\textheight
 \advance\topmargin-\headheight
 \advance\topmargin-\headsep
 \advance\topmargin-\footskip
 \divide\topmargin\tw@\botmargin\topmargin
 }%
%
\def\centerpagemargin{% calculate \oddsidemargin constrained by:
 \oddsidemargin\trimwidth
 \advance\oddsidemargin-\textwidth
 \advance\oddsidemargin-\marginparwidth
 \advance\oddsidemargin-\marginparsep
 \divide\oddsidemargin\tw@
 \evensidemargin\oddsidemargin
 \adjustpagemargin
 }%
%
\def\leftpagemargin{% calculate \oddsidemargin constrained by:
 \oddsidemargin\trimwidth
 \advance\oddsidemargin-\textwidth
 \advance\oddsidemargin-\marginparwidth
 \advance\oddsidemargin-\marginparsep
 \advance\oddsidemargin-\evensidemargin
 \adjustpagemargin
 }%

